Redesigning SLAM for Arbitrary Multi-Camera Systems

Adding more cameras to SLAM systems improves robustness and accuracy but complicates the design of the visual front-end significantly. Thus, most systems in the literature are tailored for specific camera configurations. In this work, we aim at an adaptive SLAM system that works for arbitrary multi-camera setups. To this end, we revisit several common building blocks in visual SLAM. In particular, we propose an adaptive initialization scheme, a sensor-agnostic, information-theoretic keyframe selection algorithm, and a scalable voxel-based map. These techniques make little assumption about the actual camera setups and prefer theoretically grounded methods over heuristics. We adapt a state-of-the-art visual-inertial odometry with these modifications, and experimental results show that the modified pipeline can adapt to a wide range of camera setups (e.g., 2 to 6 cameras in one experiment) without the need of sensor-specific modifications or tuning.

==> math_macros.tex <==
\newcommand{\I}{\mathtt{I}}
\global\long\def\X{\mathbf{X}}

% pose related
\newcommand{\R}{\mathtt{R}}
\newcommand{\expm}{\exp}
\DeclareMathOperator{\Expm}{Exp}
\DeclareMathOperator{\Logm}{Log}
\newcommand{\logm}{\log}
\global\long\def\se{\mathfrak{{se}}}
\global\long\def\SE{\text{{SE}}}
\global\long\def\so{\mathfrak{{se}}}
\global\long\def\SO{\text{{SE}}}

\newcommand{\expcoords}{\pmb{\theta}} % exponential coordinates of rotation
\newcommand{\expcoord}{\theta}
\newcommand{\expcoordangle}{\|\expcoords\|}
\newcommand{\pos}{\mathbf{p}}
\newcommand{\rot}{\R}
\newcommand{\vel}{\mathbf{v}}

% 3D related
\newcommand{\px}{\mathbf{u}}
\global\long\def\f{\mathbf{{f}}}
\global\long\def\pt{\mathbf{{p}}}
\global\long\def\proj{\operatorname{proj}}
\global\long\def\T{\mathtt{{T}}}

% some other useful matrices
\global\long\def\I{\mathtt{{I}}}
\global\long\def\J{\mathtt{{J}}}
\global\long\def\H{\mathtt{{H}}}
\global\long\def\F{\mathtt{{F}}}
\global\long\def\E{\mathtt{{E}}}
